Diagnosis-guided Attack Recovery for Securing Robotic Vehicles from Sensor Deception Attacks

Sensors are crucial for perception and autonomous operation in robotic vehicles (RV). Unfortunately, RV sensors can be compromised by physical attacks such as sensor tampering or spoofing. In this paper, we present DeLorean, a unified framework for attack detection, attack diagnosis, and recovering RVs from sensor deception attacks (SDA). DeLorean can recover RVs even from strong SDAs in which the adversary targets multiple heterogeneous sensors simultaneously. We propose a novel attack diagnosis technique that inspects the attack-induced errors under SDAs, and identifies the targeted sensors using causal analysis. DeLorean then uses historic state information to selectively reconstruct physical states for compromised sensors, enabling targeted attack recovery under single or multi-sensor SDAs. We evaluate DeLorean on four real and two simulated RVs under SDAs targeting various sensors, and we find that it successfully recovers RVs from SDAs in 93% of the cases.

==> sections/4-motivation.tex <==
What are the advantages of separating attack detection and diagnosis? 
Low FPs. 
Motivate probabilistic attack diagnosis over model-based attack diagnosis

What are the advantages of targeted attack recovery? Minimal disruption. 
Show an example and motivate attack diagnosis.

Which attack recovery is good for multi-sensor SDA?
Motivate designing a framework that integrates an attack detector, offers attack diagnosis, and ensures targeted attack recovery. 


==> sections/7-discussion.tex <==
\noindent
\textbf{Deployment Scenarios}
\sysname will not work in the presence of obstacles in the mission path, which is also the case for PID-Piper~\cite{pid-piper} and SSR~\cite{srr-choi}. 
RVs based on PID controller require a supplementary component in the feedback control loop and sensors such as camera and LiDAR to maneuver safely around obstacles.   
%Our experiments do not include recovery in presence of obstacles in the RV's trajectory. 
%Most industrial RVs today operate in open environments without any obstacles, \eg a drone flies hundreds of meters above the ground~\cite{dronedeliveryzipline}. 
%Techniques have been proposed to leverage geometric characteristics of the RV's trajectory and derive heading directions and optimize velocity to avoid obstacles~\cite{collision-avoid}.
%In particular, they can find a direction for avoiding the obstacle and optimize the velocity vector.  
For RV's equipped with obstacle avoidance components (including camera and LiDAR), \sysname can be extended to work with obstacle avoidance systems~\cite{collision-avoid} to adjust the heading direction and velocity leveraging the geometric characteristics of the RV's trajectory under recovery to maneuver the RV safely around obstacles.  
%Ideally, for such complex missions RVs will be equipped with obstacle avoidance systems, and \sysname can be extended to leverage the on-board obstacle avoidance system for safe recovery.
%\pritam{discuss avoidance velocoty and how obstacles can be avoided.}

\smallskip
\noindent 
\textbf{Advanced Sensors}
We evaluate \sysname on GPS, gyroscope, accelerometer, magnetometer, and barometer sensors that can be manipulated through physical attacks that inject fake signals. 
The autonomous operations in most industrial RVs today rely on the mentioned sensors~\cite{dronedeliveryzipline, dronedeliverywalmart}. %\karthik{Add citation}
Recently however, RV manufacturers have started using advanced sensors such as camera and LiDAR~\cite{wingcopter}. 
Attacks have been demonstrated targeting both the camera and LiDAR to deceive the machine learning models (ML) that are used for image classification~\cite{lidar-attack, poltergeist}.
However, these attacks are crafted for specialized ML models, and are hence out of our scope.% (different threat model assumptions). %as they have a different threat model \ie to deceive the image classification machine learning models that use camera and LiDAR feed for decision making. 

\smallskip
\noindent
\textbf{Resilient Hadware.}
Recent work has proposed a technique that leverages IMU (Inertial Measurement Unit) sensors to counteract GPS spoofing~\cite{semperfi}. 
However, this method is solely designed to mitigate GPS spoofing and is not effective against attacks targeting multiple sensors. 

